LUNA: Language Understanding with Number Augmentations on Transformers via Number Plugins and Pre-training

Transformers are widely used in NLP tasks. However, current approaches to leveraging transformers to understand language expose one weak spot: Number understanding. In some scenarios, numbers frequently occur, especially in semi-structured data like tables. But current approaches to rich-number tasks with transformer-based language models abandon or lose some of the numeracy information - e.g., breaking numbers into sub-word tokens - which leads to many number-related errors. In this paper, we propose the LUNA framework which improves the numerical reasoning and calculation capabilities of transformer-based language models. With the number plugin of NumTok and NumBed, LUNA represents each number as a whole to model input. With number pre-training, including regression loss and model distillation, LUNA bridges the gap between number and vocabulary embeddings. To the best of our knowledge, this is the first work that explicitly injects numeracy capability into language models using Number Plugins. Besides evaluating toy models on toy tasks, we evaluate LUNA on three large-scale transformer models (RoBERTa, BERT, TabBERT) over three different downstream tasks (TATQA, TabFact, CrediTrans), and observe the performances of language models are constantly improved by LUNA. The augmented models also improve the official baseline of TAT-QA (EM: 50.15 -> 59.58) and achieve SOTA performance on CrediTrans (F1 = 86.17).

==> 1-intro-old.tex <==
\label{sec:intro}

From documents and web pages to databases and data frames, table is widely used as an effective and intuitive way to store, organize and represent information. For example, \reftab{tab:A} comes from a financial report. With the abundance of tables emerge many related tasks~\cite{dong2022table}: Entity linking for tables~\citep{cutrona2020SemTab}, NL table retrieval~\citep{wang2021retrieving}, semantic parsing / text-to-SQL with tables~\citep{yu-etal-2018-spider}, question answering (QA) with tables~\citep{pasupat-liang-2015-compositional,zhu-etal-2021-tat}, table-to-text generation~\citep{chen-etal-2020-logic2text}, tabular data analysis~\citep{zhou2020Table2Analysis}, table-based fact verification~\citep{chen2020TabFact}, modeling multivariate time series~\cite{padhi2021tabular}, \etc

\begin{table}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/ExampleTAT.pdf}
    \caption{TAT-QA Example: A Financial Report Table.}
    \label{tab:A}
\end{table}

% \begin{table}[t]
%     \centering
%     \caption{TabFact Example: A Wikipedia Table.}
%     \includegraphics[width=\linewidth]{figures/ExampleTabFact.pdf}
%     \label{tab:B}
% \end{table}

% \begin{table}[t]
%     \centering
%     \caption{Credit-Fraud Example: A Transaction Table.}
%     \includegraphics[width=\linewidth]{figures/credit_fraud.pdf}
%     \label{tab:C}
%     \label{fgr: table with number}
% \end{table}

These tabular tasks require models that understand tables. Recent tabular models are developed by adding structure information and task-specific modules to language models -- especially attention-based subword-level language models. 
For example, TagOps \citep{zhu-etal-2021-tat} adopts sequence tagging by RoBERTa \citep{liu2019roberta} and symbolic reasoning with aggregation operator. 
%TaBERT \citep{yin-etal-2020-tabert} is built on top of BERT \citep{devlin-etal-2019-bert} by additional vertical self-attention over aligned row encodings, and jointly learns contextual representations for queries and tables. 
TabBERT~\citep{padhi2021tabular} is a hierarchical variant of BERT which accommodates the temporal nature of rows in the tabular input.
Similarly, TaPas \citep{herzig-etal-2020-tapas} extends BERT's architecture with structure embedding, cell selection and operator prediction.

% However, these tabular models magnifies a current weak spot in NLP -- number understanding.
% Numbers are much more common in tables comparing to general natural language texts. As we will discuss in \refsec{sec:number-stat}, \red{??.??}\% of the tables have numbers in them, and \red{??.??}\% of all table cells are numerical. The small weakness of numbers for general texts might lead to big mistakes for table-related tasks. To address this weak spot, we break it down into the following two challenges.

% First, how to properly represent a number? Recent studies show that existing number representation approaches are suboptimal and sporadic \citep{thawani-etal-2021-representing}. Existing approach to numbers either filter them out, collapse them into \texttt{[UNK]} token, or split them into arbitrary subword tokens. For example ``3.1415'' is split into ``3'', ``.'', ``14'', ``15'' by BPE \citep{sennrich-etal-2016-neural} in RoBERTa and into ``3'', ``.'', ``141'', ``\#\#5'' by WordPiece \citep{wu2016wordpiece} in TaPas and TaBERT. These approaches hardly lead to proper number representations.

% Second, how to understand a series of numbers? The structure of table naturally organize numbers successively in row or column. \red{??.??}\% of the table columns are numerical. \red{Examples of numerical field understanding in \reftab{tab:A} and \reftab{tab:B}.} The capability of understanding the semantics and statistics of a numerical field (usually column) is critical for table-related tasks.

However, these tabular models magnifies a current weak spot in language -- number understanding. Numbers are much more common in tables comparing to general natural language texts. As we will discuss in \refsec{sec:number-stat}, 97\% of the tables have numbers in them, and 54\% of all table cells are numerical. When facing tabular tasks that heavily depends on numerical reasoning and calculation (\Eg, QA, fact check, time series modelling, \etc), as we will demonstrate in \refsec{sec:tab-models}, errors could easily occur by adopting existing number representation approaches in NLP. Recent studies have already shown that these approaches are suboptimal and sporadic~\citep{thawani-etal-2021-representing}: Numbers are either filtered out, collapsed into \texttt{[UNK]} token, quantized into finite bins, or split into arbitrary subword tokens. In other words, numeracy information is abandoned or scattered around. For example ``3.1415'' is split into ``3'', ``.'', ``14'', ``15'' by BPE~\citep{sennrich-etal-2016-neural} (used in TagOps) and into ``3'', ``.'', ``141'', ``\#\#5'' by WordPiece~\citep{wu2016wordpiece} (used in TaPas).% Prevalence of numbers in tables means it would be unnecessarily hard for tabular models to understand number when they are using subword tokenizers and learning embedding representation for broken number pieces.
%Treating numbers as normal words and breaking them into sub-word tokens in a vocabulary could lead to worse performances on tabular tasks.


% We ask ourselves following questions: Are there better number representations? What are proper approach to representing numbers in NLP and tables? Can we augment existing NLP and tabular model with better number understanding capabilities?
% challenges: open vocabulary of infinite possible numbers (small to large range)

To augment the numerical reasoning and calculation capability of tabular models, we propose \textbf{TUNA} (\textbf{T}able \textbf{U}nderstanding \textbf{N}umber \textbf{A}ugmentations) framework. As shown in \reffig{fig:tuna-overview}, TUNA works as a patch for existing language models when handling rich-number tabular tasks. 

Our first key idea behind TUNA is that: \textit{Each number should be represented as a whole for model input} (rather than broken into subword tokens or quantized into binned tokens). Learning embedding representation for raw number strings properly could help capture more numeracy information for downstream tasks.
In TUNA, this idea corresponds to part I number plugin in \reffig{fig:tuna-overview}. Each number in the input (table and text) string will be first recognized by our \textbf{NumTok} (number tokenizer, see \refsec{sec:numtok}) and inserted as a special \texttt{[NUM]} token into the original input token sequence. Then, our \textbf{NumBed} (number embedder, see \refsec{sec:numbed}) encodes the raw string of the recognized number as embedding vector adding to its corresponding \texttt{[NUM]} token embedding.
%NumBed encodes a recognized number as input embedding vector to the tabular model.
%Then, to help the tabular model better understand numerical fields, various \textbf{numerical pre-training} objectives are proposed in \refsec{?}, \red{including...} Meanwhile, if the tabular model is already pre-trained before applying TUNA,

The newly introduced number embedding may be incompatible with the embedding space of the model's vocabulary tokens. To bridge the gap between number and vocabulary embedings, part II of TUNA -- \textbf{tabular pre-training} on data from downstream tasks (see \refsec{sec:tab-pretrain}) -- is designed for either starting the tabular model from scratch or from (pre-trained) checkpoint. First, to incorporate the \texttt{[NUM]} token, we modified the classical MLM (masked language model) objective with specially designed regression loss for it. Then, when starting from a checkpoint of a tabular model, it is easy for model to forget existing knowledge and overfit the downstream data. To prevent this, a teacher-student model distillation process is designed as a regularization constraint.
%to bridge the gap between the original sub-word and the additional NumBed embeddings, and prevent the model from forgetting its existing knowledge when going through new pre-training objectives.
%Finally, a tabular model with the above TUNA patches will be \textbf{fine-tuned} on down-stream tasks. \TODO{polish this paragraph}

%\TODO{Add results and hignlights to this paragraph.}
By applying TUNA to existing tabular models, we observe performance improvements on QA, fact-check and time series tasks (see \refsec{sec:results}) over four tabular models. With the help of TUNA framework, previous tabular models TagOps and TabBERT reach new SOTA numbers on TAT-QA ($EM$=59.58\% and $F1$=67.15\%) and CrediTrans ($F1$=86.17\%). By further analyze the dataset and conducting empirical studies, we further demonstrate how TUNA help preserving numeracy information for downstream tasks.

%\TODO{Summarize contributions.}
In summary, our major contributions are:
\begin{itemize}
    \item To the best of our knowledge, we are the first to point out the number understanding issues of existing tabular models.
    \item TUNA framework is proposed by us to enhance the number understanding capabilities of tabular models. The code and data of TUNA are open sourced at \url{https://anonymous.4open.science/r/TUNA-A608/}.
    \item TUNA framework to constant performance boost and SOTA, open sourced.
    \item NumTok, NumBed (first to mix string-based and real-based) choice comparisons benefits future model design and selection.
    \item Distillation and regression loss to bridge the gap between number and vocabulary embeddings.
\end{itemize}


==> 2-preliminaries-old.tex <==
\label{sec:prelim} % Ends around page 3

As discussed in \refsec{sec:intro}, number understanding is critical for table understanding. To further demonstrate this, in this section we explore the numbers from three example tabular datasets, and investigate how popular models work with them.



\subsection{Tabular Datasets and Tasks}
\label{sec:datasets}

% \begin{figure}[t]
%     \centering
%     %\includegraphics{?}
%     \caption{Question and Answers for \reftab{tab:A}.}
%     \label{fig:A}
% \end{figure}

% \begin{figure}[t]
%     \centering
%     %\includegraphics{?}
%     \caption{Statement and Results for \reftab{tab:B}.}
%     \label{fig:B}
% \end{figure}


In this paper, we take three typical table-related datasets and corresponding tasks as examples.

TAT-QA\footnote{Tabular And Textual dataset for Question Answering, \url{https://nextplusplus.github.io/TAT-QA/}} \citep{zhu-etal-2021-tat} is a recent QA dataset requiring numerical reasoning over complex and realistic tabular and textual data. In total, TAT-QA contains 16,552 questions associated with 2,757 hybrid (table + paragraphs) contexts from real-world financial reports. 20\% of the hybrid contexts are used as development and test sets. A table in TAT-QA has 3$\sim$30 rows and 3$\sim$6 columns with at least 2 human-verified relevant nearby paragraphs. We can see an example question over the hybrid context in \reftab{tab:A}.

% \TODO{delete WTQ and write about WikiTables in TabFact.}
% WTQ\footnote{WikiTableQuestions, \url{https://ppasupat.github.io/WikiTableQuestions/}} \citep{pasupat-liang-2015-compositional} is a popular but older QA dataset with only table as context for question answering. In total, WTQ contains 2,108 HTML tables from Wikipedia and 22,033 question-answer pairs generated by human. 20\% of the tables are used as development and test sets. A table in WTQ has at least 8 rows and 5 columns.

TabFact\footnote{TabFact, \url{https://tabfact.github.io/}} \citep{chen2020TabFact} is a fact verification dataset with 16k Wikipedia tables as evidence for 118k human annotated statements. In TabFact, for each Wikipedia table (with caption), the goal is to distinguish which given statements are entailed by the table and which are refuted by it. A table in TabFact has less than 50 rows and 10 columns. We can see example true and false statements over \reftab{tab:B}.

% \TODO{Add TabFormer datasets and tasks.}
CrediTrans\footnote{Credit Card Transaction Dataset, https://ibm.ent.box.com/v/tabformer-data}\citep{padhi2021tabular} is a time series corpus for credit card transactions with 24 million transactions from 20,000 users. Each transaction (row) has 12 fields (columns) consisting of both continuous and discrete attributes, such as merchant name, merchant address, transaction amount, etc.



\subsection{Exploring Numbers}
\label{sec:number-stat}

In TAT-QA, WTQ and TabFact datasets, 97.59\% of all the 30,120 tables have numbers in them (100\%, 99.93\% and 94.79\% respectively). 54.94\% of all the 2,471,520 table cells have numbers in them. (While only 17.72\% table cells contain at least 2 numbers.) When analyzing tables in row level or column levels, numbers are also hard to ignore for 71.36\% of the table columns and 85.25\% of the table rows.

%Numbers in table cells could be of high diversity. \reffig{fgr: table with number} is a non-exhaustive demonstration of this diversity.
Numbers are shown as strings in tables and texts. After ignoring edge cases, such as scientific notation, the remaining decimal number strings have clear format patterns in them: Most of them are positive numbers (0.12\% of all numbers are negative); 91.00\% and 9.00\% of all numbers are integers and float numbers, respectively; 1.51\% and 5.02\% of all numbers have percent ``\%'' or comma ``,'' character in them, respectively. % As shown in \reffig{?} (log 10 bin freq dist), \red{??.??\%} numbers fall in the range ??$\sim$????. %Context-wise, numbers could be wrapped in parentheses, coming before or after units currency symbols; Count-wise, a cell could contain zero (``N/A'', `` - \%''), one or multiple (``1.76\% - 2.50\%'') numbers.

%Numbers are shown as strings in tables and texts. As we will further discuss in \refsec{sec:numtok}, the first step to find numbers in string is to find all segments consisted by characters in ``0123456789,.+-\%''. Then within these candidate segments we manually write rules (\eg, \red{...}) to filter out non-number segments. The remaining numbers have clear format patterns in them: Most numbers are positive numbers (\red{??.??\%} of all numbers are negative) written in decimal notation rather than scientific notation ; \red{??.??\%} and \red{??.??\%} of all numbers are integers and float numbers, respectively; \red{??.??\%} and \red{??.??\%} of all numbers have percent ``\%'' or comma ``,'' character in them. \red{\etc} As shown in \reffig{?} (log 10 bin freq dist), \red{??.??\%} numbers fall in the range ??$\sim$????.

Comparing to tables, in plain texts numbers are relatively sparse. Out of 59,645 pieces of texts (including queries, paragraphs, captions) in the three datasets, there are 934,121 English words but there only 76,532 numbers in them.



\subsection{Existing Models and Number-related Issues}
\label{sec:tab-models}
As we have introduced in \refsec{sec:intro}, three very popular models -- RoBERTa, TaPas and TabBERT -- have been evaluated on the tabular datasets. RoBERTa (as the backbone of TagOps) has been evaluated on TAT-QA\citep{zhu-etal-2021-tat}, TaPas on TAT-QA and TabFact\citep{herzig-etal-2020-tapas,zhu-etal-2021-tat}, and TabBERT on CrediTrans\citep{padhi2021tabular}. 

The common practice of language models and tabular models usually adopt a fixed vocabulary and the sub-word tokenization approaches like BPE\citep{sennrich-etal-2016-neural} and WordPiece\citep{Wu2016GooglesNM} in the tokenizer. Instead of considering the number as an ensemble, the tokenizer splits the number into arbitrary tokens. 
From another perspective, TabBERT\citep{padhi2021tabular} quantifies numbers into buckets by their value. This might be a good attempt, but loses the information of similarity between nearby numbers in different buckets. 

As we have discussed in \refsec{sec:intro}, breaking a number into sub-word pieces or quantifying it is not a grounded practice. 
% In comparison, breaking a word into sub-word pieces has linguistic supports 
% \cite{?}
% and experimental supports 
% \cite{?}
% .
%The diversity that numbers can be presented in raises challenges for number processing pipelines to correctly recognize the existence and set boundaries for numbers.
Beyond the example of ``3.1415'' in \refsec{sec:intro}, we can find more counter-intuitive results yield by subword-level tokenizers.
For instance, ``1.76\%-2.50\%'' is splitted into [``0'', ``.'', ``76'', ``\%'', ``-'', ``2'', ``.'', ``50'', ``\%''] by BPE and WordPiece, where the number count (2 rather than 4 numbers) and boundaries (between 0.76\% and 2.50\%) are unclear, and the distinction between numerical symbols (decimal point / minus sign) and grammatical punctuation marks (period / hyphen) is hindered.
In fact, the numerical information of numbers is usually neglected in language models and tabular models since the model vocabulary is usually based on the statistical property of the common corpus without giving special attention to numbers. For example, TaPas uses BERT vocabulary where among 30,522 tokens, only 3.48\% of them are plain numbers. More strikingly, all these plain number tokens are integer, and 96.98\% of them are within 2,000. Unfortunately, the scarcity and imbalanced distribution of number tokens are hard to solve by simply enlarging the model vocabulary. As an enhancement of the original BERT model, Roberta enlarges the vocabulary to 50,000 using byte-level BPE, but only 3.36\% tokens contain numbers. Different from the common practice described above, TabBERT quantizes continuous fields to build its own finite vocabulary to better capture real number information. Although quantization is a highly effective method in number processing, the exact values are still lost.

% \TODO{Hongwei: write about model errors}
For the TAT-QA input case mentioned in \reftab{tab:A}, the original Roberta tags at ``\$2,082'' and ``\$2,025'', operates ``CHANGE\_RATIO'' to them and returns ``0.0281''. This is because, the model is confused by the segment, ``percentage change in interest expense'', in the question. The error show that the model lacks the ability to understand numbers and correlate numbers to text. When seeing the word ``percentage change'', the model arbitrarily filters the same-number pairs. 
% \TODO{Polish this paragraph of error analysis.}
% With numbers represented by arbitrary tokens and with pre-train objectives mainly designed for natural language subwords, these three models start to act weirdly on number-related samples. \red{For example, } in \reffig{?} we can see that TagOps ... on \reftab{tab:A}. In reffig{?} TaPas predicts both statements as entailed while they only have number differences... on \reftab{tab:B}... One root cause of these number-related errors is that BPE (used by RoBERTa) and WordPiece (used by TaBERT and TaPas) split numbers into arbitraty subword tokens. \red{\Eg}, in \reftab{tab:A} cell ``....''...




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




\subsection{Table-related Tasks}
There are a line of table-related tasks, requiring substantial understanding of the table content. TableQA \citep{zhu-etal-2021-tat} \citep{chen-etal-2021-finqa} \citep{yang-etal-2018-hotpotqa} and Table Fact Verification \citep{chen2020TabFact} are two representative Table-related tasks. In recent years, more interest has been drawn to the intersection between tables and natural language generation \citep{suadaa-etal-2021-towards}\citep{chen-etal-2021-de}\citep{li-etal-2021-improving-encoder}\citep{su-etal-2021-shot-table}. 
% \cite{dong2022table}


\subsection{Tabular Models}
Tabular models are often pretrained on large-scale unsupervised tables or table-query pairs \citep{iida-etal-2021-tabbie}\citep{herzig-etal-2020-tapas}\citep{yin-etal-2020-tabert}\citep{eisenschlos-etal-2021-mate}. TaPas \citep{herzig-etal-2020-tapas} and TaBERT \citep{yin-etal-2020-tabert} are two representative tabular models. Recently tabular model survey papers \cite{dong2022table} have also emerged, profiling and summarizing different aspects of the tabular model spectrum.
% \citep{chen-etal-2020-logical}



\subsection{Numeracy in NLP}
In the NLP field, a significant amount of effort has been put into finding high-quality representations for numbers. The task is usually to encode numbers into an emebdding.  \citep{thawani-etal-2021-representing} 
Some previous work has been touching on number distributions\citep{spithourakis-riedel-2018-numeracy} \citep{elazar-etal-2019-large}. However, they tend to be utilizing distributions only to model single numbers, instead of querying semantics contained in the distribution itself. Some previous work also explored the effect of number magnitude \citep{spithourakis-riedel-2018-numeracy}. Within the realm of Natural Language, DROP \citep{dua-etal-2019-drop} is a representative dataset bringing up numeracy challenges.



% \subsection{Table pretrain}
% \TODO{Hongwei} Table pretrain

% Refer our pre-train survey paper \cite{dong2022table}

